NaSGEC: a Multi-Domain Chinese Grammatical Error Correction Dataset from Native Speaker Texts

We introduce NaSGEC, a new dataset to facilitate research on Chinese grammatical error correction (CGEC) for native speaker texts from multiple domains. Previous CGEC research primarily focuses on correcting texts from a single domain, especially learner essays. To broaden the target domain, we annotate multiple references for 12,500 sentences from three native domains, i.e., social media, scientific writing, and examination. We provide solid benchmark results for NaSGEC by employing cutting-edge CGEC models and different training data. We further perform detailed analyses of the connections and gaps between our domains from both empirical and statistical views. We hope this work can inspire future studies on an important but under-explored direction--cross-domain GEC.

==> figures/anno_performance.tex <==
\begin{figure}[t!]
\centering
\includegraphics[scale=0.45]{pictures/anno_performance_pic.pdf}
\caption{The distributions of Top-10 most frequent error types on each domain of MD-CGEC and MuCGEC.}
\label{fig:error:dis}
\end{figure}

==> figures/data_num.tex <==
\begin{figure}[tb!] %插入图片
\centering %图片居中
\scalebox{0.8}{
\begin{tikzpicture}
\begin{axis}[
    legend style={
                fill opacity=2,
                legend cell align={left},
                text=black,
                at={(0.44,0.35)},
                anchor=north west,
                font=\small,
              },
    xlabel={\textbf{Proportion of used fine-tuning data}},
    ylabel={\textbf{F$_{2}$}},
    ylabel style = {yshift=-10pt},
    ymin=30, ymax=50,
    symbolic x coords={25\%,50\%,75\%,100\%},
    xtick=data,
    % ytick={40,...,50},
    ymajorgrids=true,
    xmajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=midnightblue!80,thick, dashdotted,
    mark=square*,
    mark options={solid,mark size=2pt}
    ]
    coordinates {
    (25\%,41.17)(50\%,42.71)(75\%,44.22)(100\%,45.48)
    };
    \addlegendentry{Baseline (\textsc{Media})}

\addplot[
    color=midnightblue!80, thick,
    mark=triangle*,
    mark options={solid,mark size=2pt}
    ]
    coordinates {
    (25\%,44.21)(50\%,45.29)(75\%,45.93)(100\%,46.64)
    };
    \addlegendentry{Adaptation (\textsc{Media})}

\addplot[
    color=brickred!80,thick, dashdotted,
    mark=diamond*,
    mark options={solid,mark size=2pt}
    ]
    coordinates {
    (25\%,38.21)(50\%,39.78)(75\%,40.50)(100\%,41.81)
    };
    \addlegendentry{Baseline (\textsc{Thesis})}

\addplot[
    color=brickred!80, thick,
    mark=pentagon*,
    mark options={solid,mark size=2pt}
    ]
    coordinates {
    (25\%,42.09)(50\%,42.60)(75\%,43.33)(100\%,43.75)
    };
    \addlegendentry{Adaptation (\textsc{Thesis})}
    
    
\end{axis}
\end{tikzpicture}
}

\caption{
Impact of domain adaptation with different proportions of used fine-tuning data.
}
\label{fig:data:num}
\end{figure}

==> tables/anno_performance.tex <==
\begin{center}
\begin{table}[!t]
\centering
\scalebox{0.75}{
\begin{tabular}{cccc}
\toprule
 \textbf{Metric} & \textbf{\textsc{Media}} & \textbf{\textsc{Thesis}} \\ \hline
\textbf{Det. Consistency Ratio} & 72.12 & 82.76  \\
\textbf{Cor. Consistency Ratio} & 33.19 & 38.95  \\
\textbf{Annotation Accuracy} & 72.54$_{\pm 8.31}$ & 75.19$_{\pm 6.77}$ \\
\bottomrule
\end{tabular}
}
\caption{Annotation analysis. ``Det.'' and  ``Cor.'' means detection and correction, respectively.
} 
\label{tab:anno:performance}
\end{table}
\end{center}
\vspace{-1.0cm}

==> tables/data_exp_f0.5.tex <==
\begin{table}[t]
\centering
\scalebox{0.58}{
\begin{tabular}{ccccccccc}
\toprule
\textbf{Test $\rightarrow$}   & \multicolumn{2}{c}{\textbf{\textsc{Media}}} & \multicolumn{2}{c}{\textbf{\textsc{Thesis}}} & \multicolumn{2}{c}{\textbf{\textsc{Exam}}} & \multicolumn{2}{c}{\textbf{CCTC}} \\
\textbf{Train $\downarrow$}  & \textbf{F$_{2}$}        & \bigtriangleup            & \textbf{F$_{2}$}         & \bigtriangleup           & \textbf{F$_{2}$}      & \bigtriangleup & \textbf{F$_{2}$}      & \bigtriangleup           \\ \midrule

\textbf{\textit{Baseline}}  & 45.54       & ---       & 29.23        & ---       & 11.04      & ---  & 21.94      & ---       \\ \hdashline
\textbf{\textsc{Media}}  & \textbf{45.48}       & \textbf{+ 14.28}       & 39.72        & + 7.65        & 8.25      & -- 2.79  & 20.80     & -- 1.14       \\
\textbf{\textsc{Thesis}} & 36.04       & + 4.84        & \textbf{41.81}        & \textbf{+ 9.74}        & 9.79      & -- 1.25   & 23.85      & + 1.91       \\
\textbf{\textsc{Exam}}   & 27.47       & -- 3.73        & 28.59        & -- 3.43        & \textbf{26.91}      & \textbf{+ 15.87}     & 19.15      & -- 2.79    \\

\textbf{CCTC}   & 33.21       & + 2.01       & 31.83        & + 2.60       & 7.12      & -- 3.92     & \textbf{45.69}      & \textbf{+ 9.59}    \\ \bottomrule
\end{tabular}
}
\caption{Domain transfer performance. $\bigtriangleup$ denotes the relative improvements over corresponding baselines.}
\label{tab:transfer}
\end{table}

==> tables/data_exp_other_datasets.tex <==
\textbf{
\begin{table*}[t!]
\centering
\scalebox{0.8}{
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
% & \multicolumn{3}{c}{\textbf{NaMuDom}}                     & \multirow{2}{*}{\textbf{CCTC}} & \multirow{2}{*}{\textbf{FCGEC}} & \multirow{2}{*}{\textbf{NLPCC18}} & \multirow{2}{*}{\textbf{MuCGEC}} \\ \cmidrule{2-4}
 & \multicolumn{3}{c|}{\textbf{CCTC}}    & \multicolumn{3}{c|}{\textbf{FCGEC}}  & \multicolumn{3}{c}{\textbf{MuCGEC}} \\ 
% \hline
& \textbf{P} & \textbf{R} & \textbf{F$_{0.5}$} & \textbf{P} & \textbf{R} & \textbf{F$_{0.5}$} & \textbf{P} & \textbf{R} & \textbf{F$_{0.5}$} \\ \midrule
% \multicolumn{10}{c}{\textbf{\textit{One stage training}}}   \\ 
\textbf{\textit{Previous SOTA}}                                                                        & 35.19 & 28.40 & 33.58 &  48.19 & 37.14 & 45.48 & \textbf{54.69} & 29.10 & \textbf{46.51}  \\ \midrule
\textbf{Real Learner}   & 8.35 & 46.56 & 9.99 & 33.50  & 10.93 & 23.71 & 53.77 & 28.58 & 45.71  \\
\textbf{Pseudo Native}  & 19.41 & 45.99 & 21.94 & 7.35 & 0.55 & 2.12 & 49.57 & 9.79 & 27.35 \\
% \midrule
% \multicolumn{10}{c}{\textbf{\textit{Two stage training}}}   \\ 
\textbf{Pseudo Native $\Rightarrow$ Real Learner} & 9.12 & 49.26 & 10.90 & 33.33 & 10.46 & 23.19 & 53.84 & \textbf{29.77} & 46.34\\
\textbf{Real Learner $\Rightarrow$ Pseudo Native} & 19.29 & 43.62 & 21.71  & 4.90 & 0.39 & 0.48 & 47.12 & 8.49 & 24.66  \\ \midrule
\textbf{Best + Fine-tuning} & \textbf{47.36} & \textbf{46.97} & \textbf{47.28} & \textbf{55.88} & \textbf{44.62} & \textbf{53.19} & -- & -- & -- \\
\bottomrule
\end{tabular}
}
\caption{Benchmark results on previous CGEC datasets. ``Best + Fine-tuning'' means that for each dataset, we further fine-tune our best system in the second major row on the corresponding training set (MuCGEC is an exception since it is just an evaluation dataset without the training set).}
\label{tab:data:exp:other}
\end{table*}}
\vspace{-0.5cm}


% \textbf{\begin{center}
% \begin{table*}[t!]
% \scalebox{0.6}{
% \begin{tabular}{lccccccc}
% \hline
% % & \multicolumn{3}{c}{\textbf{NaMuDom}}                     & \multirow{2}{*}{\textbf{CCTC}} & \multirow{2}{*}{\textbf{FCGEC}} & \multirow{2}{*}{\textbf{NLPCC18}} & \multirow{2}{*}{\textbf{MuCGEC}} \\ \cmidrule{2-4}
% & \textbf{NaMuDom (\textsc{Media})}    & \textbf{NaMuDom (\textsc{Thesis})}   & \textbf{NaMuDom (\textsc{Exam})}     & \textbf{CCTC}                               &     \textbf{FCGEC}                            &          \textbf{NLPCC18}                         &     \textbf{MuCGEC}                             \\ 
% % \hline
% & \textbf{P/R/F$_{2}$}    &\textbf{P/R/F$_{2}$}   & \textbf{P/R/F$_{2}$}     & \textbf{P/R/F$_{2}$}                               &     \textbf{P/R/F$_{2}$}                            &     \textbf{P/R/F$_{0.5}$}                              & \textbf{P/R/F$_{0.5}$}                                 \\ \hline
% \multicolumn{8}{c}{\textbf{\textit{One stage training}}}   \\ 
% \textbf{R. L.}                                                                        & 35.96/29.15/30.30 & 24.16/34.06/31.48 & 23.01/11.31/12.58  & 8.35/46.56/24.31                & 33.50/10.93/12.63               & 48.97/32.80/44.58                 & 53.77/28.58/45.71                \\
% \textbf{P. N.}                                                                       & 53.39/29.17/32.08 & 30.86/33.52/32.95 & 9.78/2.60/3.05    & 19.41/45.99/36.10              & 7.35/0.55/0.67                  & 56.51/13.30/34.25                 & 49.57/9.79/27.35                 \\ \hline
% \multicolumn{8}{c}{\textbf{\textit{Two stage training}}}   \\ 
% \textbf{P. N. $\Rightarrow$ R. L.} & 38.37/31.16/32.38 & 25.67/35.09/32.69 & 24.48/11.59/12.95 & 9.12/49.26/26.20               & 33.33/10.46/12.12               & 49.62/34.43/45.60                 & 53.84/29.77/46.34                \\
% \textbf{R. L. $\Rightarrow$ P. N.} & 51.90/26.20/29.08 & 31.61/31.97/31.90 & 10.77/2.52/2.98   & 19.29/43.62/34.83              & 4.90/0.39/0.48                  & 55.12/10.34/30.58                 & 47.12/8.49/24.66                 \\ \hline
% \end{tabular}
% }
% \caption{Experimental results (Precision/Recall/F-value) based on BART with different training data on NaMuDom and other CGEC benchmarks. R.L. denotes Real Learner training data, and P. N. means Pseudo Native training data.}
% \label{tab:data:exp}
% \end{table*}
% \end{center}}
%

==> tables/domain_transfer_2.tex <==
\begin{table}[t]
\centering
\scalebox{0.65}{
\begin{tabular}{cccc}
\toprule
\textbf{Test $\rightarrow$}   & \textbf{\textsc{Media}} & \textbf{\textsc{Thesis}} & \textbf{\textsc{Exam}} \\
\textbf{Train $\downarrow$}  & \textbf{P/R/F$_{0.5}$} & \textbf{P/R/F$_{0.5}$} & \textbf{P/R/F$_{0.5}$} \\ \midrule
\textbf{\textsc{Media}}  & \textbf{61.35/42.72/56.43}     & 32.73/41.07/34.12       & 20.71/5.08/12.82      \\
\textbf{\textsc{Thesis}} & 53.22/32.95/47.39       & \textbf{34.96/43.96/36.45}     & 19.95/5.14/12.66  \\
\textbf{\textsc{Exam}}  & 36.98/17.56/30.29  & 18.89/21.17/19.31          & \textbf{48.29/24.23/40.29}   \\ \bottomrule
\end{tabular}
}
\caption{Results for fine-tuning experiments.}
\label{tab:transfer}
\end{table}


==> tables/domain_transfer_f0.5.tex <==
\begin{table}[t]
\centering
\scalebox{0.58}{
\begin{tabular}{ccccccccc}
\toprule
\textbf{Test $\rightarrow$}   & \multicolumn{2}{c}{\textbf{\textsc{Media}}} & \multicolumn{2}{c}{\textbf{\textsc{Thesis}}} & \multicolumn{2}{c}{\textbf{\textsc{Exam}}} & \multicolumn{2}{c}{\textbf{CCTC}} \\
\textbf{Train $\downarrow$}  & \textbf{F$_{0.5}$}        & \bigtriangleup            & \textbf{F$_{0.5}$}         & \bigtriangleup           & \textbf{F$_{0.5}$}      & \bigtriangleup & \textbf{F$_{0.5}$}      & \bigtriangleup           \\ \midrule

\textbf{\textit{Baseline}}  & 45.54       & ---       & 29.23        & ---       & 17.57      & ---  & 21.94      & ---       \\ \hline
\textbf{\textsc{Media}}  & \textbf{56.43}       & \textbf{+ 10.89}       & 33.60        & + 4.37        & 15.09      & -- 2.48  & 20.80     & -- 1.14       \\
\textbf{\textsc{Thesis}} & 47.21       & + 1.67        & \textbf{36.45}        & \textbf{+ 7.22}        & 17.44      & -- 0.13   & 23.85      & + 1.91       \\
\textbf{\textsc{Exam}}   & 41.06       & -- 4.48        & 28.59        & -- 0.64        & \textbf{40.29}      & \textbf{+ 22.72}     & 19.15      & -- 2.79    \\

\textbf{CCTC}   & 48.49      & + 2.95       & 31.83        & + 2.60       & 12.20      & -- 5.37     & \textbf{31.16}      & \textbf{+ 9.22}    \\ \bottomrule
\end{tabular}
}
\caption{Domain transfer performance. $\bigtriangleup$ denotes the relative improvements over corresponding baselines.}
\label{tab:transfer}
\end{table}
